On the Possibilities and Limitations of Multi-hop Reasoning Under Linguistic Imperfections

Systems for language understanding have become remarkably strong at overcoming linguistic imperfections in tasks involving phrase matching or simple reasoning. Yet, their accuracy drops dramatically as the number of reasoning steps increases. We present the first formal framework to study such empirical observations. It allows one to quantify the amount and effect of ambiguity, redundancy, incompleteness, and inaccuracy that the use of language introduces when representing a hidden conceptual space. The idea is to consider two interrelated spaces: a conceptual meaning space that is unambiguous and complete but hidden, and a linguistic space that captures a noisy grounding of the meaning space in the words of a language---the level at which all systems, whether neural or symbolic, operate. Applying this framework to a special class of multi-hop reasoning, namely the connectivity problem in graphs of relationships between concepts, we derive rigorous intuitions and impossibility results even under this simplified setting. For instance, if a query requires a moderately large (logarithmic) number of hops in the meaning graph, no reasoning system operating over a noisy graph grounded in language is likely to correctly answer it. This highlights a fundamental barrier that extends to a broader class of reasoning problems and systems, and suggests an alternative path forward: focusing on aligning the two spaces via richer representations, before investing in reasoning with many hops.

==> UNUSED/old_step2.tex <==
We will use the following lemma to characterize the distance between a fixed node-pair in random graphs: 
\begin{lemma}[Minimum distances in random graphs, Lemma 1 of \citet{chung2002average}]
\label{lemma:max:dist:vol}
In a random graph $G$ 
% in $G(\mathbf{w})$
with a given expected degree sequence $\mathbf{w} = (\degA(1), \hdots, \degA(n))$, for any fixed pair of nodes $(u, v)$, the distance $d(u, v)$ between $u$ and $v$ is greater than
$\floor{  \frac{ \log \vol{G} - c }{ \log \tilde{\text{deg}} }  }$  with probability at least
\[
1 - \frac{ \degA(u) \degA(v) }{ \tilde{\text{deg}} (\tilde{\text{deg}} - 1) } e^{-c}.
\]
\end{lemma}

In this lemma, the volume of the graph is defined to be the sum of the node degrees, i.e., 
$\vol{G} =  \sum_i \degA(i)$. $\tilde{d}$ is the second-order average degree, defined by $\tilde{\text{deg}} = \sum \degA(i)^2 \big/ \sum \degA(i)$. 


\begin{lemma}\label{lem:UBthm1}
    If $\lambda \ball(d))^2 p_- \leq \frac{1}{2 e n}$, then 
    $\prob{ s \pathk{\leq \tilde{d}} s' \mid m \npathk{} m' }
      \leq \prob{ \text{dist}(v_s,v_{s'}) \leq \tilde{d} }
      \leq \frac{1}{\sqrt{n}}.$
\end{lemma}
\begin{proof}

{
\color{red}

\[
\prob{ s \pathk{\leq \tilde{d}} s' } = 
% \prob{\cup_p E_p}
\prob{ \bigvee_{\ell=1, \cdots, \tilde{d}} s \pathk{ \tilde{d}} s' }
\leq \sum_{\ell\leq \tilde{d}} { n \choose \ell} \tilde{p}^\ell
\leq \sum_{\ell\leq \tilde{d}} (\frac{e n}{\ell})^\ell \tilde{p}^\ell
%  \leq \tilde{d}e n \tilde{p}\leq c . 
\]

\[
\leq \sum_{\ell\leq \tilde{d}} ({e n})^\ell \tilde{p}^\ell
\leq 
{e n\tilde{p}}\frac{
        ({e n\tilde{p}})^{\tilde{d}}-1
    }{
        {e n\tilde{p}}-1
    }
\leq \frac{e n\tilde{p}}{1-e n\tilde{p}}    
\leq 2 e n\tilde{p}. 
\]
Assume $\tilde{p}\leq \frac{1}{2 e n}$.
}





To identify the upper bound on $\prob{ s \pathk{\leq \tilde{d}} s' | m \npathk{} m' } $, recall the definition of \(\tilde{G}_S\), given an instance of $G_S$ 
(as outlined in Lemmas~\ref{lemma:graph:homogination2} and~\ref{lemma:graph:homogination}, for 
$\tilde{p} = \lambda \ball(d))^2 p_-$).
Lemma~\ref{lemma:graph:homogination} relates the connectivity of $s$ and $s'$ to a connectivity event in \(\tilde{G}_S\), i.e., \( \prob{ s \pathk{\leq \tilde{d}} s' \mid m \npathk{} m' } \leq \prob{\text{there is a path from $v_s$ to $v_{s'}$ in $\tilde{G}_S$ with length } \tilde{d} }\), where $v_s, v_{s'}\in V_{\tilde{G}_S}$ are the nodes corresponding to the components containing $s$ and $s'$ respectively. Equivalently, in the following, we prove that the event $\text{dist}(v_s,v_{s'})\geq \tilde{d}$ happens with a significant probability.

% We model the probability that there would be no path between disconnected nodes in the symbol-graph. 
% Since $G_S$ is non-homogeneous its analysis could be difficult. 
% We use Lemma~\ref{lemma:graph:homogination} and Lemma~\ref{lemma:graph:homogination2} to transform the analysis to a homogeneous graph $\tilde{G}(n, \tilde{p})$, where $\tilde{p} = (\lambda \ball(d))^2 \cdot p_- $. 


Lemma~\ref{lemma:max:dist:vol} provides a lower-bound probability of existence of paths between any fixed pair of nodes $u$ and $v$. We use this lemma for $v_s$ and $v_{s'}$. 
Note that the volume of the graph $\vol{G} = n^2\tilde{p}$ and second-order average degree $\tilde{\text{deg}}= n \tilde{p}$. Then, we have:


\begin{equation}
\label{eqn:upper-bound}
  \prob{ \text{dist}(v_s,v_{s'}) < \frac{ \log (n^2 \tilde{p}) - c }{ \log (n \tilde{p} ) } } \leq \Theta(1) e^{-c}.
\end{equation}
\ashish{The asymptotic $\Theta$ notation above is somewhat confusing, as it's unclear what happens to it when we go to the expression below for $c = 1/2$. It seems to have disappeared. let's make the constant explicit, rather than asymptotic.}
Choose $c = \frac{1}{2}\log n$: 
% \begin{align*}
%     \prob{ dist(s, s')   \geq \frac{ \log (n^2 \tilde{p}) - \frac{1}{2} \log n }{ \log (n \tilde{p} ) } } \geq 1 - \frac{1}{\sqrt{n}}.
% \end{align*}

% \begin{align*}
%     \Rightarrow \prob{ dist(s, s')   \geq \frac{ 1.5\log (n) - \log \frac{1}{\tilde{p}} }{ \log (n \tilde{p} ) } } \geq 1 - \frac{1}{\sqrt{n}}
% \end{align*}


\begin{align*}
    \prob{ \text{dist}(v_s,v_{s'}) < \frac{\log (n^{1.5}\tilde{p})}{\log (n\tilde{p})} } \leq \frac{1}{\sqrt{n}}.
\end{align*}
One can verify that \(\frac{\log (n^{1.5}\tilde{p})}{\log (n\tilde{p})}> \tilde{d}\), when \((n\tilde{p})^{\tilde{d}-1}\leq 1\).
Therefore assuming \(n\tilde{p}\leq 1\) (or, $p_- \cdot \ball^2(d)  \leq \frac{1}{\lambda n}$), we have:
\begin{equation*}
    \prob{ \text{dist}(v_s,v_{s'}) \leq \tilde{d} }
      \leq \frac{1}{\sqrt{n}} \nonumber
\end{equation*}
%
Applying Lemma~\ref{lemma:graph:homogination}, we obtain:
\begin{equation}
    \prob{ s \pathk{\leq \tilde{d}} s' \mid m \npathk{} m' }
      \leq \prob{ \text{dist}(v_s,v_{s'}) \leq \tilde{d} }
      \leq \frac{1}{\sqrt{n}}.
\end{equation}
\end{proof}


==> UNUSED/oldstuff/old-proofs.tex <==
\begin{lemma}[Neighborhood size in a random graph, Lemma 3 of \cite{bollobas1981diameter}]
\label{lemma:neighborhood:size}
For a random graph $\renymodel$, define $\Gamma_d$ to be the set of nodes at distance $d$ from a fixed node. 
Let $K \geq 11$ be a constant, and define 
$$
\alpha_d = K \sqrt{ \frac{ \log n }{ (pn)^d } }
$$
$$
\beta_d = p (pn)^{d-1} 
$$
$$
\gamma_d = \frac{2(pn)^{d-1}}{n}
$$
$$
\delta_d = \exp \left( 2\sum_{l = 1}^d (\alpha_l + \beta_l + \gamma_l ) \right)  - 1 
$$

For sufficiently large $n$, with probability at least $1 - n^{-K - 2}$ for every vertex $x$ and every natural number $d$ smaller than the graph diameter: 

$$
\left| |\Gamma_d|  - (pn)^d  \right| \leq \delta_d (pn)^d
$$
\end{lemma}



\todo{explain what these proofs are here. }

\begin{proof}[Proof of Lemma~\ref{lemma:lower-bound}]
Let $pt$ be the path in the symbol graph corresponding to path connecting $m$ and $m'$ in the meaning graph:  
\begin{align*}
 \mathbb{P} & \big( s \pathk{k,d} s'  \Big| m \eone m' \big) \\
& \geq \mathbb{P} 
  \begin{bmatrix}
    \text{for an arbitrary path $pt$ and value }k' (k'\geq k)\\
    \text{all clusters in $pt$ are bigger than }k' \text{ and there is}\\
    \text{at least $k$ edges between adjacent cluster pairs} 
  \end{bmatrix}
  \\
& = \prod_{v\in pt} \prob{|\oracle(v)|\geq k'} \\ 
& \hspace{0.7cm} \cdot \prod_{(v,u)\in pt} \prob{|E(\oracle(v),\oracle(u))|\geq k \Big|~ |\oracle(v)|,|\oracle(u)|\geq k'} \\
& = \left(1-F_h(k')\right)^d \cdot \left(1 - F_{\bin{k'^2,p_+}}(k) \right)^{d-1}.
% & = (1-F_h(k'))^d \cdot \left(\sum_{i=k}^{+\infty} {k'^2\choose i}p_+^i(1-p_+)^{k'^2-i}\right)^{d-1}.  \\
\end{align*}
\todo{define the notation $E$; and comment out the definition for matching }
In the second step, the inequality 
is due to ignoring noisy edges. The RHS probability only considers an event based on factual edges in the second line which is a subset of first line event.
\end{proof}

% {
% \color{red}
% $$
% \sigma_{2}(L) \leq \frac{x^T L x}{x^Tx} \leq \sigma_{\max}(L)
% $$

% Cluster: $G(k', p_+)$ with Laplacian $L$
% Cluster $G(k', 1-p_+)$ with Laplacian $L^c$
% $L^c = K_{k'}- L$


% $\sigma_{2}(L) = k'-1 - \sigma_{\max}(L^c)$

% }


\begin{proof}[Proof of Lemma \ref{lemma:upper-bound}]
We assume $m$ and $m'$ are disconnected.
%there is at least a cut disconnecting the two components that each contain $m$ and $m'$. 
Within each of the components, the $d$-neighborhood of each node are at most $\ell \leq \ball(m, d)$ and $\ell' \leq  \ball(m', d)$. 
\begin{align*}
\mathbb{P}[ s \pathk{k,d} s'  & | m \etwo m' ] \\
&  \leq \mathbb{P} 
  \begin{bmatrix}
    \text{at least $k$ noisy edges between two } \\ 
    \text{components are added in } G_S\\
  \end{bmatrix} \\ 
% P[\text{at least $k$ noisy edges between two components are added in } G_S ]\\
& = 1-F_{\bin{\ell\cdot\ell',p_- }}(k) \\
% & = \sum_{i=k}^{+\infty} {\ell\cdot\ell'\choose i}p_-^i(1-p_-)^{n-i}. \\
\end{align*}
\end{proof}

\begin{comment}
{
\color{red}
Here we bound $\ell$:  
\begin{align*}
\mathbb{P}[ s \pathk{k,d} s'  & | m \etwo m' ] \\
&  \leq \mathbb{P} 
  \begin{bmatrix}
    \text{at least $k$ noisy edges between two } \\ 
    \text{components are added in } G_S\\
  \end{bmatrix} \\ 
&  = \sum_{\ell} \mathbb{P} 
  \begin{bmatrix}
    \text{at least $k$ noisy edges between two } \\ 
    \text{components are added in } G_S | component size\\ 
  \end{bmatrix} \prob{\text{connected component is } \ell } \\ 
% & = \sum_{i=k}^{+\infty} {\ell\cdot\ell'\choose i}p_-^i(1-p_-)^{n-i}. \\
\end{align*}


\begin{align*}
\mathbb{P}[ s \pathk{k,d} s'  & | m \etwo m' ] \\
&  \leq k\mathbb{P} 
  \begin{bmatrix}
    \text{one noisy edges between two } \\ 
    \text{components of } s, s' \\
  \end{bmatrix} + 
  k \mathbb{P} 
  \begin{bmatrix}
    \text{two noisy edges between }s \text{ or } s' \\ 
    \text{to one of the components }\\
  \end{bmatrix} + 
  k \mathbb{P} 
  \begin{bmatrix}
    \text{three noisy edges} \\ 
    \text{between the two nodes } s, s' \\ 
  \end{bmatrix} 
  \\ 
&  
\leq  k \cdot \ell\cdot\ell' \cdot p_-   
+ k \cdot n \cdot p_-^2 \cdot (\ell + \ell') 
+ k \cdot n^2 \cdot p_-^3 
\end{align*}
}
\end{comment}

\begin{proof}[Proof of Theorem~\ref{the:reasoning:possiblity}]
% We show the result holds 
% For what values of $d, \alpha, p, p_+, p_-$? 
% Selection of the parameters: 
% $$p_- = \log n / n $$
% $$k' = \lambda $$
% $$p_+ = (1 - \epsilon)^{1/\lambda}$$
% $$ *** $$
% If the latent event is $ m \pathk{d} m'$, first we show that the probability of observing a $\lambda,d$ path in the symbol graph is lower-bounded by some constant, for small values of $d$ (Lemma~\ref{lemma:lower-bound}). 
% In a similar fashion, we show that, 
% if the latent event is $ m \npathk{d} m'$, 
% the probability of observing a $\lambda,d$ path in the symbol graph is upper-bounded by some constant, for small values of $d$ (Lemma~\ref{lemma:upper-bound}). 
% With proves that it is possible to distinguish which of the latent events have happened given the surface information, with probability at least 0.5. 
Based on the results of Lemma~\ref{lemma:lower-bound} and Lemma~\ref{lemma:upper-bound}, 
if we prove that the following inequalities hold,
% \begin{align*}
% \max_{k': k' \geq k}\Big[  \left(1-F_h(k')\right)^d \cdot  (1 -  & F_{\bin{k'^2,p_+}}(k) )^{d-1} \Big] \\ 
% & > 1-F_{\bin{B^2(d),p_- }}(k)
% \end{align*}

$$
\begin{cases}
 \left(1-F_h(k')\right)^d \cdot \left(1 - F_{\bin{k'^2,p_+}}(k) \right)^{d-1}  & >  c_1  \\ 
1-F_{\bin{B^2(d),p_- }}(k) & <  c_2 
\end{cases}
$$
an algorithm which looks for $k,d$ connectedness in the symbol graph would have a performance strictly bigger than $\min\{c_1, 1-c_2\}$.\footnote{
The true-positive probability is at least $c_1$ and the true-negative probability is at least $1-c_2$. Depending on the distribution of positive and negatives, one of the constants will dominate the performance. $\min \{ c_1, 1-_c2 \}$ is a lower-bound to a any data distributions. 
}



Since our goal is to show the \emph{possibility} of such algorithm, we simply prove that the inequalities for $c_1 = c_2 = 0.5$  given the selection of the parameters in Theorem~\ref{the:reasoning:possiblity}. 
In our proof we choose the node sampling distribution to be a Poisson with parameter $\lambda = k' + 2$. 
% Rather than showing this, we show that there is a constant $c \in (0, 1)$ such that: 

As for sampling probabilities $p_+$ is a positive constant close to one, and $p_- = \frac{\log n}{n}$. We start with the first inequality: 
$$
A(k, k', p_+, d) = \left(1-F_h(k')\right)^d \cdot \left(1 - F_{\bin{k'^2,p_+}}(k) \right)^{d-1} > c 
$$
Rather than optimizing it for $k'$ we set its valued to a reasonable number. In our setting we use: 
$$k = k' \left( 1 - (1-p_+)^{k'^2} \right) $$
The intuition behind this selection is that for: (a) the size of the matching is at most $k'$ and it is achieved when $p_+$ is almost close to 1. (b) the size of the matching shrinks for smaller $p_+$ and gets to almost zero, for $p_+ = 0$. There is a more rigorous analysis on the size of matching we refer the interested  readers to the work of \namecite{frieze2012maximum}. 
We show that for any $\lambda \geq 4$, $p_+ \geq 0.5$ and $d \leq 3$:  
$$
A(k, k', p_+, d) > 0.05
$$
First note that the function is decreasing with $d$, and increasing with $\lambda$ and $p_+$. Hence, for the given range, the minimum is achieved for $(d, \lambda, p_+) = (3, 4, 0.5)$, which is $0.0501$.

% To keep things simple we make further approximations, but for tighter conditions. 
% In other words, we find the parameters for the tighter inequality,
% as long as it is not going to violate the inequality. For example in this case, since the value inside parenthesis is smaller than 1, we can use a smaller value for the power, and not violate the constraint: 
% $$
% \left(1-F_h(k')\right)^{d} \cdot \left(1 - F_{\bin(k'^2,p_+)}(k) \right)^{d} > c 
% $$
% $$
% \Rightarrow \left(1-F_h(k')\right) \cdot \left(1 - F_{bin(k'^2,p_+)}(k) \right) > c^{1/{d}} 
% $$
% $$
% 1-F_h(k') - F_{bin(k'^2,p_+)}(k) > c^{1/d} 
% $$

% $$
% 1-  c^{1/d} > F_h(k') + F_{bin(k'^2,p_+)}(k)
% $$

% $$
% 1-  c^{1/d} >  \frac{(1+k') \cdot e^{-k}  \cdot k^k }{k!}  + (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{ck^2 - k}
% $$


Next we consider the upper-bound term: 
$$
\ball(d, p_-) = 1-F_{\bin{B^2(d),p_- }}(k) < c 
$$
$$
\Rightarrow \ball(d, p_-) = (k+1) (1-p_-)^{B^2(d)} < c 
$$

The noisy edge sampling parameter is $p_- = \log n \big/ n$ and the ball assumption is defined as $\ball(d) = \zeta^d$. We show that for any $n \geq 10^6$, $d \leq 3$ and $\zeta \leq 7$, the inequality is satisfied. 
This function is increasing with $d$ and $\zeta$, and decreasing with $n$, hence the maximum is achieved where $(d, n, \zeta) = (3, 10^6, 6)$, and it is $0.0043$. 


% $$
% \Rightarrow F_{bin(B^2(d),p_- )}(k) > 1-c 
% $$
% $$
% \Rightarrow (k+1) (1-p_-)^{B^2(d)}  > 1-c
% $$
% $$
% \Rightarrow \ball(d)   < \sqrt {  \log \frac{1-c}{k+1} \Big/\log (1-p_-)  } 
% $$
% $$
% \Rightarrow \ball(d) = \zeta^d  \Rightarrow \zeta{^{d_0}}  \leq \sqrt {  \log \frac{1-c}{k+1} \Big/\log (1-p_-)  } 
% $$
% $$
% \Rightarrow d_0   \leq \frac{1}{\log \zeta} \log \sqrt {  \log \frac{1-c}{k+1} \Big/\log (1-p_-)  } 
% $$
% $$
% d_0   \leq \frac{1}{\log \zeta} \log \sqrt {  \log \frac{1-c}{k+1} \Big/\log \frac{n - \log n}{n}  } 
% $$
% $$
% \ball(d) = d^\tau  \Rightarrow d_0  \leq  \left\lbrace  \log \frac{1-c}{k+1} \Big/\log (1-p_-)  \right\rbrace^{\tau /2}
% $$
% $$***$$

$$
\frac{ (1+k') \cdot e^{-\lambda}  \cdot \lambda^{k'} }{k'!} + (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{k'^2 - k}  < c 
$$

\begin{comment}
We factor out $k!$ in the denominator: 

$$
1-  c^{1/d} > \frac{1}{k!} \left[  (1+k') \cdot e^{-k}  \cdot k^k   + (1+k) \frac{ {k'}^2! }{ ({k'}^2 - k)! } {p_+}^{k} (1-p_+)^{ck^2 - k} \right] 
$$

Use sterling approximation for factorials: 
$$
1-  c^{1/d} > \frac{1}{k!} \left[  (1+k') \cdot e^{-k}  \cdot k^k   + (1+k) 
\frac{{k'}}{ \sqrt{ {k'}^2 - k} } 
\left( \frac{{k'}^2}{e} \right)^{{k'}^2}  \left( \frac{{k'}^2 - k}{e} \right)^{-({k'}^2 - k)} 
{p_+}^{k} (1-p_+)^{ck^2 - k} \right] 
$$

Simplify $e^.$ together: 
$$
1-  c^{1/d} > \frac{1}{k!} \left[  (1+k') \cdot e^{-k}  \cdot k^k   + (1+k) 
e^{k}
\frac{{k'}}{ \sqrt{ {k'}^2 - k} } 
\frac{ {k'}^{2{k'}^2} }{  ({k'}^2 - k)^{ ({k'}^2 - k) }  }
{p_+}^{k} (1-p_+)^{ck^2 - k} \right] 
$$


Replace the assumption $p_+ = (1-\epsilon)^{1/\lambda}$ and assume that $p_+$ is close to 1. 
With this assumption: ${p_+}^{k} = 1-\epsilon$ and $(1-p_+)^{ck^2 - k} = s$
$$
1-  c^{1/d} > \frac{1}{k!} \left[  (1+k') \cdot e^{-k}  \cdot k^k   + (1+k) 
e^{k}
\frac{{k'}}{ \sqrt{ {k'}^2 - k} } 
\frac{ {k'}^{2{k'}^2} }{  ({k'}^2 - k)^{ ({k'}^2 - k) }  }
{p_+}^{k} (1-p_+)^{ck^2 - k} \right] 
$$

Replace Sterling and use Matlab: 

$$
\frac{
1/2^{50*k + 1/2}*3060513257434037^k*\left(
k^k*\exp{(-k)}*(kp + 1) + 
\frac{
(2^(50*k)/3060513257434037^k*p^k*(k + 1)*(kp^2)^(kp^2 + 1/2)*(1 - p)^(kp^2 - k))
}{
(kp^2 - k)^{(kp^2 - k + 1/2)}
} 
\right)
} { 
k^{k + 1/2}*\pi^{1/2}
}
$$

Assume that $p+$ is big and hence $k = k'$: 

% {
% \color{red}

$$
\left(1-d \cdot F_h(k')\right) \cdot \left(1 - (d-1)F_{\bin{k'^2,p_+}}(k) \right) > 1-F_{\bin{B^2(d),p_- }}(k)
$$


$$
1-d \cdot F_h(k') - (d-1)F_{\bin{k'^2,p_+}}(k)  + d(d-1)F_h(k') F_{\bin{k'^2,p_+}}(k)  > 1-F_{\bin{B^2(d),p_- }}(k)
$$

$$
d \cdot F_h(k') + (d-1)F_{\bin{k'^2,p_+}}(k) < F_{\bin{B^2(d),p_- }}(k)
$$

$$
d \cdot e^{-\lambda} \cdot \sum_{i=0}^{k'} \frac{ \lambda^{i} }{ i! }  + (d-1) \left(\sum_{i=0}^{k} {k'^2 \choose i} p_+^{i} (1-p_+)^{k'^2 - i} \right)  < 
\sum_{i=0}^k { B^2(d) \choose i } p_-^i (1-p_-)^{B^2(d) - i}
$$

With approximate the RHS with a lower-bound, and the LHS with an upper-bound:  
\begin{align*}
\frac{d \cdot (1+k') \cdot e^{-\lambda}  \cdot \lambda^{\lambda} }{\lambda!}   + (d-1) (1+k) \max & \left\lbrace {k'^2 \choose k} p_+^{k} (1-p_+)^{k'^2 - k}, {k'^2 \choose k'^2p_+}  p_+^{k'^2p_+} (1-p_+)^{k'^2 (1 - p_+)}  \right\rbrace  \\
& \hspace{1cm} <  (k+1) \min \left\lbrace  { B^2(d) \choose k } p_-^k (1-p_-)^{B^2(d) - k}, (1-p_-)^{B^2(d)} \right\rbrace 
\end{align*}

$$
\frac{d \cdot (1+k') \cdot e^{-k}  \cdot k^k }{k!}  + (d-1) (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{ck^2 - k} < 
(k+1) (1-p_-)^{B^2(d)} 
$$


$$
\frac{1}{(k+1)} \left[ \frac{ d \cdot (1+k') \cdot e^{-k}  \cdot k^k }{k!}  + (d-1) (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{ck^2 - k} \right] < 
 1-B^2(d) p_-
$$

$$
B^2(d) < \frac{1}{p_-} \left\{ 1 -  \frac{1}{(k+1)} \left[ \frac{ d \cdot (1+k') \cdot e^{-k}  \cdot k^k }{k!}  + (d-1) (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{ck^2 - k} \right] \right\}
$$
% }


% {
% \color{blue}

$$
\log \left\{ \frac{1}{(k+1)} \left[ \frac{d \cdot (1+k') \cdot e^{-k}  \cdot k^k }{ k!}  + (d-1) (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{k'^2 - k} \right]  \right\} <  B^2(d) \log (1-p_-) 
$$

Note that $\log (1-p_-) < 0$: 
$$
B^2(d)  < \frac{1}{\log (1-p_-) } \log \left\{  \frac{1}{(k+1) } \left[ \frac{d \cdot (1+k') \cdot e^{-k}  \cdot k^k }{ k!}  + (d-1) (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{k'^2 - k} \right]   \right\}
$$

$$
B^2(d)  < \frac{ 1 }{\log (1-p_-) } \log \left\{ \frac{ d - 1 }{(k+1) } \left[ \frac{ (1+k') \cdot e^{-k}  \cdot k^k }{ k!}  + (1+k) {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{k'^2 - k} \right]    \right\}
$$


We replace $(1+k')$ with $(1+k)$, since $k < k'$: 
$$
B^2(d)  < \frac{ 1 }{\log (1-p_-) } \log \left \{ (d - 1) \left[ \frac{ e^{-k}  \cdot k^k }{ k!} + {{k'}^2 \choose k} {p_+}^{k} (1-p_+)^{k'^2 - k} \right]    \right\}
$$

$$
B^2(d)  < \frac{ 1}{ \log (1-p_-) } \log \left\{ \frac{ d - 1 }{ k! } \left[ e^{-k}  \cdot k^k + \frac{{k'}^2!}{ ({k'}^2 - k)! } {p_+}^{k} (1-p_+)^{k'^2 - k} \right]    \right\}
$$


$$
B^2(d)  < \frac{ 1}{ \log (1-p_-) } \log \left\{ \frac{ d - 1 }{ k! } \left[ e^{-k}  \cdot k^k + \frac{{k'}}{ \sqrt{ {k'}^2 - k} } 
\left( \frac{{k'}^2}{e} \right)^{{k'}^2}  \left( \frac{{k'}^2 - k}{e} \right)^{-({k'}^2 - k)}  {p_+}^{k} (1-p_+)^{k'^2 - k} \right]   \right\}
$$

% }


% {
% \color{gray}

$$*** $$

$$
\log \log n \cdot (1+k \sqrt{c}) \left( \frac{e^{-k}  \cdot k^k }{k!}  + {ck^2 \choose k} (c/k)^{k} (1-(c/k))^{ck^2 - k} \right)  < 
(k+1) (1-\alpha^{2\log n}/n) 
$$

$$
\alpha  < \left[  
 n \left( 1- \frac{\log n \cdot (1+k \sqrt{c})}{(k+1)} \left( \frac{e^{-k}  \cdot k^k }{k!}  + {ck^2 \choose k} (c/k)^{k} (1-(c/k))^{ck^2 - k} \right) \right) \right]^{-2\log n}
$$

Using Sterling 
$n! \sim \sqrt{2 \pi n}\left(\frac{n}{e}\right)^n$: 


$$
\alpha  < \left[  
 n \left( 1- \frac{\log n \cdot (1+k \sqrt{c})}{(k+1)} \left( \frac{e^{-k}  \cdot k^k }{\sqrt{2\pi k} (k/e)^k }  + {ck^2 \choose k} (c/k)^{k} (2 -c^2k)) \right) \right) \right]^{-2\log n}
$$

$$
\alpha  < \left[  
 n \left( 1- \frac{\log n \cdot (1+k \sqrt{c})}{(k+1)} \left( \frac{1}{\sqrt{2\pi k}  }  + {ck^2 \choose k} (c/k)^{k} (2 -c^2k)) \right) \right) \right]^{-2\log n}
$$

$$
\alpha  < \left[  
 n \left( 1- \frac{\log n \cdot (1+k \sqrt{c})}{(k+1)} \left( \frac{1}{\sqrt{2\pi k}  }  + \frac{c^k}{k^{ck^2}}{ck^2 \choose k}(k - c)^{k(ck - 1)} \right) \right) \right]^{-2\log n}
$$

Using sterling for the 2nd term: 
$$
{ck^2 \choose k} (c/k)^{k} (1-(c/k))^{ck^2 - k} = (1/(0.3)^k*2^(1/2)*c^k*(1 - c/k)^(c*k^2 - k))/(2*k^(2*k + 1/2)*pi^(1/2))
$$

$$
{ck^2 \choose k} (c/k)^{k} (1-(c/k))^{ck^2 - k} = 
\frac{(3.3c)^k k^{- 2 k} (1 + c - c^2 k)}{\sqrt{2 \pi k}}
$$

$$
\alpha  < \left[  
 n \left( 1- \frac{\log n \cdot (1+k \sqrt{c})}{(k+1)} \left( \frac{1  + (3.3c)^k k^{- 2 k} (1 + c - c^2 k) }{\sqrt{2\pi k}  } \right) \right) \right]^{-2\log n}
$$

$$
\alpha  < \left[  
 n \left( 1-  (\log n \cdot \sqrt{c}) \frac{1  + (3.3c)^k k^{- 2 k} (1 + c) }{\sqrt{2\pi k}  } \right) \right]^{-2\log n}
$$


$$
\alpha  < \left[  
 n^{-2\log n} \left( 1+ 2 (1 + c) \sqrt{c} \log^2 n \frac{1  + (3.3c)^k k^{- 2 k}  }{\sqrt{2\pi k}  } \right) \right]
$$


$$
\alpha  < 
 n^{-2\log n} O\left( \log^2 n \Big/ k^{2 k+ 0.5}  \right) 
$$

if $k = \log n$ => 
$n = e^k$ 
$k^k = \log n^{\log n} = \log n (\log \log n)$

$$
\alpha  < 
 n^{-2\log n} O\left( \log n \Big/ \log \log n  \right) 
$$
% }
\end{comment}
\end{proof}

% { 
% \color{red}
\begin{proof}
We want to formalize the probability that there would be a jump between the clusters: 
\begin{align}
\prob{ s \pathk{2} s' | m \pathk{1} m'} & \geq \prob{\text{direct edge}} +  \prob{
\text{jump to one of the neighbors of } s \text{, and then connect to }s'}  \\ 
& = p_+ + 1-[1-\epsilon_+ p_+]^{k'-1} - p_+ \left(1-[1-\epsilon_+ p_+]^{k'-1} \right)
\end{align}

$$
\prob{ s \pathk{2} s' | m \pathk{1} m'} \geq  1 - (1- p_+) \left(\epsilon_+ p_+ \right)^{k'-1} 
$$


We want to formalize the probability that there is a path of size at most $2d$: 
$$
\prob{ s \pathk{2d} s' | m \pathk{d} m'} \geq \left( \prob{ s \pathk{2} s' | m \pathk{1}  m'} \right)^{ d } \geq \left(  1 - (1- p_+) \left(\epsilon_+ p_+ \right)^{k'-1}  \right)^d
$$

$$
\prob{ s \pathk{4} s' | m \pathk{2} m'} \geq  
$$




Note that this is conditioned on the fact that the size of the clusters are $\geq k'$. We distribute the probabilities: 
$$
\begin{cases}
P_{Pois(\lambda)} (X \geq k') \geq \delta_4 \\ 
\left(  1-  (1-\epsilon_+)^{k'-1}(1-p_+)^{k'}  \right)^d \geq \delta_5
\end{cases}
$$

With tail inequalities we have: 
$$
P(X \leq \lambda / e) \leq \exp(-\lambda)  \exp(2 + \frac{\lambda}{e}) = \exp (-\lambda (1-1/e)+2 )
$$

$$
\Rightarrow P(X \geq \lambda / e) \geq 1- \exp (-\lambda (1-1/e)+2 ) \geq \delta_4
$$

$$
\Rightarrow \lambda \geq \frac{ 2 + \log \frac{1}{1-\delta_4} }{1-1/e}  
$$

If we assume that $\epsilon_+ = p_+$: 
$$
\epsilon_+ = p_+ \geq  \left( 1 - \log^{1/d} \frac{1}{\delta_5} \right)^{1 \big/ 2k'-1}
$$

And: 
$$
\delta_4 \delta_5 = \delta \Rightarrow  \delta_4 = \delta_5 = \sqrt{\delta}
$$

Next we model the probability that there would be no path between disconnected nodes. Assume that there is a cut disconnecting the two nodes $m$ and $m'$. We show that the corresponding cut in the surface graph has a zero size with a high probability. 
$$
\prob{ s \npathk{} s' | m \npathk{} m'} \geq \delta
$$


First define the following events: 
$$
\begin{cases}
e_1 = \text{there would be no noise edge between two components, each of size } \ell  \\ 
e_2 = \text{each node $s, s'$ is connected to a component of size at most } \ell \\ 
e_3 = \text{each node cluster in the surface graph has size less than } k''
\end{cases}
$$
And note that we have: 
$$
\prob{ s \npathk{} s' | m \npathk{} m'} \geq \prob{e_1|e_2, e_3} \prob{e_2 | e_3} \prob{e_3}  
$$

We provide lower-bounds for each of the above probabilities. For the first event $e_1$ we have: 
\begin{align}
& \prob{e_1 = \text{there would be no noise edge between two components, each of size } \ell   }  = (1-p_-)^{\ell^2} \geq \delta_1
\end{align}
% $$
% \prob{ s \pathk{2} s' | m \npathk{} m'} \leq \prob{\text{each node $s, s'$ is connected to a component of size at most }\ell} =1- (1-p_-)^{\ell^2} \leq 1-\delta_1
% $$
$$
(1-p_-)^{\ell^2} \geq \delta \Rightarrow e^{-\ell^2 p_-} \geq \delta_1 \rightarrow \ell  \leq \sqrt{ \frac{\delta_1}{p_-} }
$$


Next we characterize $\ell$ in terms of $\ball(d)$, $k''$, $p_-$. Assuming that $p_+$ is high, a given node is likely to be connected to all the $k'' \cdot \ball(d)$ nodes it was already connected too. To this we will add the nodes that are connected because of the node $p_-$. Using Lemma~\ref{lemma:max:neighbood:size} we know that, with probability at least $1-o(n^{-1})$: $ |N(d)|  \leq 2d^3 (\log n + d \log \log n) $. Hence the following choice of neighborhood size holds: 
$$
\prob{\ell \leq k'' \cdot \left( \ball(d) + 2d^3 (\log n + d \log \log n)  \right)  } \geq 1 - 1/n \geq \delta_2
$$

This upperbound on the neighborhood size, we get an upperbound on the ball-assumption: 
$$
k'' \cdot \left[ \ball(d) + 2d^3 (\log n + d \log \log n)  \right] \leq \sqrt{ \frac{\delta_1}{p_-} } \Rightarrow
 \ball(d) \leq \frac{1}{k''} \sqrt{ \frac{\delta_1 \cdot n}{\log n} } - 2d^3 (\log n + d \log \log n)
$$
$$
1 - \frac{1}{n} \geq \delta_2 \Rightarrow n \geq \frac{1}{1-\delta_2}
$$

% Note that this is assuming that the size of the cluster. 
Next we formulate the probability distribution of $e_3$. Another part of this distribution has to be from the fact that the clusters have of size at most some constant. We distribute the rest of the probability there using  Lemma~\ref{lemma:poisson:bound}. Given $\lambda$, pick $k'' = c \mu $ then: 
$$
P(X \geq c\lambda) \leq \frac{ e^{ \lambda (c-1) } }{ c^{c\lambda} } \Rightarrow P(X < c\lambda) \geq 1 - \frac{ e^{ \lambda (c-1) } }{ c^{c\lambda} }
$$

And we have to make sure: 
$$
1 - \frac{ e^{ \lambda (c-1) } }{ c^{c\lambda} } \geq \delta_3 \Rightarrow \lambda \leq  \frac{1 }{ c (\log c - 1) + 1 } \log \frac{1}{1 - \delta_3}
$$
And we have to make sure that: 
$$
\delta_1 \delta_2 \delta_3 = \delta \Rightarrow \delta_i = \delta^{1/3}
$$

To have a feasible solution: 
$$
\frac{ 2 + \log \frac{1}{1-\delta_4} }{1-1/e} = 3.16 + 1.58 \frac{1}{1-\delta_4}   \leq \lambda \leq  \frac{1 }{ c (\log c - 1) + 1 } \log \frac{1}{1 - \delta_3}
$$



% \todo{Distribute the probability mass between the two events. }

% $$
% \begin{cases}
% \prob{ s \pathk{2} s' | m \npathk{} m'} \leq 1 - \delta_1  \\ 
% P_{Pois(\lambda)} (X \leq k") \geq \delta_1 \\
% P (\ell \leq N(d)) \geq 1 - 1/n \geq \delta_2 
% \end{cases}
% $$
\end{proof}

%% Old proofs: 


\begin{comment}


\todo{write the proof for this}

\begin{lemma}[Chernoff bound for Poisson distribution]
\label{lemma:poisson:bound}
Bounds for the tail probabilities of a Poisson random variable $ X \sim \operatorname{Pois}(\lambda)$ can be derived using a Chernoff bound argument: 
$$
P(X \geq x) \leq \frac{e^{-\lambda} (e \lambda)^x}{x^x}, \text{ for } x > \lambda
$$
$$
P(X \leq x) \leq \frac{e^{-\lambda} (e \lambda)^x}{x^x}, \text{ for } x < \lambda.
$$
\end{lemma}


\begin{lemma}[Chung and Lu, Lemma 1]
\label{lemma:max:neighbood:size}
Suppose $np > 1$. With probability at least $1-o(n^{-1})$ we have: 
$$
|N(d)| \leq 2d^3 \log n (np)^d
$$
for any $d \in [1, n]$. 
\end{lemma}

\end{comment}




\begin{lemma}
\label{lemma:neighborhood:size:our:graph}
For a random graph $\renymodel$, define $\Gamma_d$ to be the set of nodes at distance $d$ from a fixed node. 
If $pn = \log n$ then the size of the neighborhood is at least 
$$
(\log n)^d  \left( 2 - \exp \left( \frac{K}{ \log^{(d-1)/2} n } \right)   \right) \leq \Gamma_d(x)
$$
where $K$ is a constant bigger than 22. 
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:neighborhood:size:our:graph}]
According to Lemma~\ref{lemma:neighborhood:size} we know: 
$$
\left| |\Gamma_d|  - (\log n)^d  \right| \leq \delta_d \log^d n
$$

from which the $\Gamma_d$ size can be lower-bounded: 
$$
 (\log n)^d  (1-\delta_d) \leq \Gamma_d
$$

Now we have to find an upper-bound for $\delta_d$. If $pn = \log n$: 
$$
\alpha_d = K \sqrt{ \log^{-(d-1)} n }
$$
$$
\beta_d = p \log^{d-1}n
$$
$$
\gamma_d = \frac{2\log^{d-1} n}{n}
$$
$$
\delta_d = \exp \left( 2\sum_{l = 1}^d \left(  K \sqrt{ \log^{-(l-1)} n } + \frac{ 2}{n} \log^{l}n  + \frac{2\log^{l-1} n}{n} \right) \right) - 1 
$$
$$
\delta_d = \exp \left(  2K \sum_{l = 1}^d  \log^{-(l-1)/2} n  + 
\frac{4}{n} \sum_{l = 1}^d  \log^l n  + 
\frac{4}{n} \sum_{l = 1}^d \log^{l-1} n \right) - 1 
$$
Using Geometric series: 
% $$
% \delta_d = \exp \left(  2K \sum_{l = 1}^d  \log^{-(l-1)/2} n  + 
% \frac{4}{n} \sum_{l = 1}^d  \log^l n  + 
% \frac{4}{n} \sum_{l = 1}^d \log^{l-1} n \right) - 1 
% $$
% Using Jensen's inequality if $X$ is a random variable and $\varphi$ is a convex function, then
% $$
% \varphi \left(\operatorname {E} [X]\right)\leq \operatorname {E} \left[\varphi (X)\right].
% $$
$$
\delta_d = \exp \left(  2K \frac{  \log^{-d/2} n  - 1 }{ \log^{-1/  2} n - 1  } + 
\frac{4}{n} \log n \frac{\log^{d+1} n - 1}{\log n - 1}   + 
\frac{4}{n} \frac{ \log ^d n - 1  }{ \log n - 1 }  \right) - 1 
$$
for big values of $n$:
$$
\delta_d = \exp \left( \frac{2K}{ \log^{(d-1)/2} n } + 
\frac{4\log^{d+1} n }{n}   + 
\frac{4\log^{d-1} n  }{ n }  \right) - 1 
$$
and 
$$
\delta_d \leq  \exp \left( \frac{2K + 2}{ \log^{(d-1)/2} n } \right) - 1 
$$
$$
1 - \delta_d \geq  2 - \exp \left( \frac{2K + 2}{ \log^{(d-1)/2} n } \right) 
$$

% { 
% \color{blue}
% Using Taylor series, if $x$ is small: 
% $$
% e^{x} \approx 1 + x 
% $$
% $$
% \delta_d \approx  \frac{2K}{ \log^{(d-1)/2} n } + 
% \frac{4\log^{d+1} n }{n}   + 
% \frac{4\log^{d-1} n  }{ n }
% $$
% For big values of $n$: 
% $$
% \delta_d \leq   \frac{2K + 2}{ \log^{(d-1)/2} n } \in 1+ O \left( \frac{1}{ \log^{(d-1)/2} n }\right)
% $$
% }

% {
% \color{gray}
% $$
% \delta_d = \pro d_{l = 1}^d \left[ \exp \left(2K \log^{-(l-1)/2} n \right) \cdot \exp \left(  \frac{ 2}{n} \log^{l}n \right) \cdot 2 \exp \left( \frac{\log^{l-1} n}{n} \right) \right] - 1
% $$
% }
% $$
% \delta_d = \prod_{l = 1}^d \left[  n^{-K(l-1)} \cdot n^{2p(l-1)}  \cdot \exp \left( \frac{\log^{l-1} n^2}{n} \right) \right] - 1 
% $$
$$
(\log n)^d  \left( 2 - \exp \left( \frac{2K + 2}{ \log^{(d-1)/2} n } \right)   \right) \leq \Gamma_d(x)
$$
which concludes our result. 
% $$
% (pn)^d = n \Rightarrow d0 = \log n / \log (pn) = \log n / \log \log n 
% $$
% }
\end{proof}

\begin{lemma}
\label{lemma:neighbor:as:distance}
For a random graph $\renymodel$, define $\Gamma_d$ to be the set of nodes at distance $d$ from a fixed node. Similarly, $N_d$ is the size of the the $d$-neighborhood, i.e. $N_d = \cup_{i = 1}^n \Gamma_i$. Then, $N_d = \Gamma_{d+1}$, for $d > 2$. 
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lemma:neighbor:as:distance}]
Assuming that there is a tree with which one can traverse and visit the neighbors. 
It is enough to notice that the size of the internal nodes in the tree is the same as the size of the leaf nodes. 
\end{proof}


% \begin{lemma}
% For a bipartite graph with $2n$ nodes, $n$ on each side, we put a random edge between each node pairs with probability $p$. The expected size of the matching is: 
% $$
% n \left( 1 - (1-p)^{n^2} \right)
% $$
% \end{lemma}
% \begin{proof}
% Define the bipartite graph to be collection of $n$ nodes on the right (R) and on the left (L). For each node on the left, the probability that it will be connected to at least one of the $k$ nodes on the right is $1 - (1-p)^k$.  
% \end{proof}



\begin{lemma}
\label{lemma:simplification}
For any positive values $p, \delta \in (0, 1)$, it can be shown that: 
$n \cdot p ^{n-1} \leq \delta$, 
for any $n \geq \max \left\lbrace  \frac{8}{\delta \log^2 \frac{1}{p} }, 2 \right\rbrace$. 
\end{lemma}
\begin{proof}
For simplicity, define $p= e^{-y}$ (i.e. $y = \log \frac{1}{p}$). Now consider:
\begin{align*}
n p^{n-1} = n e^{-y(n-1)}=\dfrac{n}{e^{y(n-1)}} = 
\dfrac{n}{1+ y(n-1)+ y^2(n-1)^2/2 + \cdots } \\ 
\leq \dfrac{2n}{y^2(n-1)^2} \leq 
\dfrac{2n}{y^2(n/2)^2} = \dfrac{8}{ny^2} \leq \delta.
\end{align*}
In the previous simplifications we used the fact that $n-1 \geq n/2$, for $n \ge 2.$

We conclude that $n_0 > (1/\delta)(8/y^2) = (1/\delta)\left(8\big/(\log \frac{1}{p})^2\right)$. 
\end{proof}

% \begin{lemma}
% The random-graph connectivity probability $P_n$ (Lemma~\ref{ref:connectivity:graph}) is strictly increasing, for $n \geq 2$. 
% \end{lemma}
% \begin{proof}
% To prove this we show that the difference $P_n - P_{n-1} > 0$:  
% \begin{align*}
%     P_n - P_{n-1} & = 
%     \left( 1-\sum\limits_{i=1}^{n-1}P_i{n-1 \choose i-1}(1-p)^{i(n-i)} \right) - 
%     \left( 1-\sum\limits_{i=1}^{n-2}P_i{n-2 \choose i-1}(1-p)^{i(n-i-1)} \right) \\
%     & = \left( \sum\limits_{i=1}^{n-2}P_i{n-2 \choose i-1}(1-p)^{i(n-i-1)} \right) - 
%     \left( \sum\limits_{i=1}^{n-1}P_i{n-1 \choose i-1}(1-p)^{i(n-i)} \right) \\
%     & = \sum\limits_{i=1}^{n-2}P_i{n-2 \choose i-1}(1-p)^{i(n-i-1)} \left[ 1 - \frac{n-1}{n-i} \cdot (1-p)^i \right] -  P_{n-1} \cdot (1-p)^{n-1} 
% \end{align*}

% \end{proof}

\begin{lemma}[Hoeffding bound for Binomial Distribution]
\label{lemma:haeffding}
Define the lower-tail probability of a Binomial distribution as following: 
$$
F_{\bin{n, p}}(k) = \prob{ X \leq k}= \sum_{i=0}^{k} \binom{n}{i} p^i (1-p)^{n-i}
$$
for some $\varepsilon > 0$, Hoeffding's inequality bounds the tail probability: 
$$
\prob{ X \leq (p-\varepsilon) n }
\leq\exp\left(-2\varepsilon^2 n\right)
$$
in a similar fashion, the upper-tail probability can be written as following:
$$
\prob{X \geq (p+\varepsilon)n}\leq\exp\left(-2\varepsilon^2 n\right).
$$
\end{lemma}

\begin{theorem}
\label{the:reasoning:possiblity}
For any meaning graph with $n > 10^5$ nodes, if the sampling of the nodes is done with a Poisson distribution with parameter $\lambda > 5.5$, 
positive edge sampling rate $p_+$ a constant probability bigger than $0.7$, 
noisy edge sampling rate $p_- = \log n\big/ n$, 
ball assumption $\ball(d) = \zeta^d$ ($\zeta \leq 5$),
it is possible to distinguish the two events  $m \pathk{d} m'$ vs $m \npathk{} m'$ with probability strictly greater than 0.5, for $d \leq 3$.  
\end{theorem}


Before proving this theorem, we provide two key lemmas. In each of these lemmas we provide approximate bounds to the probability of observing a $(k,d)$-path in the symbol graph, given any of the events in the meaning graph. The proof of each lemma is included in the appendix.

\begin{lemma}
\label{lemma:lower-bound}
For fixed pair of nodes $m,m'\in V_M$, and arbitrary $s\in \oracle(m)$, $s'\in \oracle(m')$, the probability that $s,s'$ are $(k,d)$-connected, for any $k, d \in \mathbb{Z}^+$, assuming that there is a path of length $d$ between $m$ and $m'$, is at least $\left(1-F_h(k')\right)^d \cdot \left(1 - F_{\bin{k'^2,p_+}}(k) \right)^{d-1}$, for any $k' \in [k, +\infty)$. 
\end{lemma}

% While there are may be many ways to accomplish the decision rule in Equation~\ref{eq:decision}, we make 

\begin{lemma}
\label{lemma:upper-bound}
For a fixed pair of nodes $m, m'\in V_M$, and arbitrary $s\in \oracle(m)$, $s'\in \oracle(m')$, the probability that 
$(s,s')$ are $(k,d)$-connected, assuming that $m$ and $m'$ are disconnected, is at most 
$
1-F_{\bin{\left(\ball(m)\cdot \ball(m'),p_- \right)}}(k)
$
\end{lemma}

With the necessary lemmas introduced, we give a high-level proof of Theorem~\ref{the:reasoning:possiblity}, and leave the details to the Appendix. 


\begin{comment}
\begin{lemma}[Connectivity of a random graph~\cite{gilbert1959random}]
\label{ref:connectivity:graph}
Denote the probability of a random undirected graph $\renymodel$ being connected with $P_n$. We can expand this formula as following: 
$$
P_n = 1-\sum\limits_{i=1}^{n-1}P_i{n-1 \choose i-1}(1-p)^{i(n-i)}
$$
\end{lemma}

\begin{proof}
It suffices to show that
$$
\sum_{i=1}^n {n-1 \choose i-1} P_i (1-p)^{i(n-i)} = 1,
$$
since ${n-1 \choose n-1}P_n(1-p)^{n(n-n)}=f(n).$ Let $v_1, v_2, \ldots, v_n$ be $n$ vertices. Trivially,
$$
1= \sum_{i=1}^n \prob{v_1 \text{ is in a component of size }i}.
$$
Now let's consider why 
$$
\prob{v_1 \text{ is in a component of size }i}={n-1\choose i-1}\prob{G(i,p) \text{ is connected} } (1-p)^{i(n-i)}.
$$

If $A$ is the set of all $i-1$ subsets of $\{v_2, v_3, \ldots, v_n\}$, then 
\begin{align*}
\prob{v_1 \text{ in comp of size }i} &= \sum_{A \in \mathcal{A}}  \prob{ \text{the comp of }v_1\text{ is }\{v_1\}\cup A} \\&=  
\sum_{A \in \mathcal{A}}  \prob{\{v_1\}\cup A \text{ is conn'd}}  \prob{\text{no edge btwn }A\cup\{v_1\} \& \ (A\cup \{v_1\})^c }.
\end{align*}

This last equality is due to the fact that the edges within $\{v_1\}\cup A$ are independent of the edges from $A$ to $A^c$. There are precisely ${n-1 \choose i-1}$ elements in $\mathcal{A}$. The probability that $\{v_1\}\cup A$ is connected is equal to the probability that $G(1+|A|,p)$ is connected, which is $f(i)$. There are $i(n-i)$ missing edges from $\{v_1\}\cup A$ to $(\{v_1\}\cup A)^c$. 
\end{proof}
\end{comment}



\begin{theorem}
\label{th:impossible}
Let $m,m'\in G_M$ be two nodes from meaning graph, connected with a path of distance at most $d$. Given a cut $C$ between $m$ and $m'$, from which $G_M'$ is constructed by deleting the edges included in $C$. Denote the symbol graphs of $G_M$ and $G_M'$, with $G_S$ and $G_S'$, respectively. 
Suppose in the sampling, the positive edge sampling $p_+$  is a positive constant bigger than $p_-$ and $p_- \geq c \log n \big/ n$ for some constant $c$. 
If $L$ and $L'$ are the Laplacian matrices corresponding to the $d(1+\lambda)$-neighbourhood of $m$, in $G_S$ and $G_S'$, and $d > \log n$: 
$$\frac{\|L-L'\|_2}{\|L\|_2} \overset{P}{\rightarrow} 0$$
for any $\ball(n) \in o(n^{1/4})$ and big enough $n$. 
% where $\varepsilon$ is a small positive number smaller than $(1/n)^d$. 
%  the ball assumption $\ball(d) = \zeta^d$, for some positive constant $\zeta$
% % where $|C|$ is the number of edges in the cut, 
% where $d$ is the distance between $m-m'$ in $G_M$, and $n$ the number of nodes in the meaning graph. 
% Also, let $d$ and $c$ be the distance and minimum cut between $s$ and $t$ in $G_M$. Finally, let $L$ denote the Laplacian matrix corresponding to the $d$-neighbourhood of $s$ in symbol graph corresponding to $G_M$. Similarly, $L'$ is the Laplacian matrix of a graph defined on the set of nodes as $L$, however the edges in the cut $C$ are sampled according to $bern(p_-)$ (instead of $bern(p_+)$ as in $G_S$). We have:
\end{theorem}

% \todo{where is the effect of the node duplication? I think it should apprear in the denominator}
